$K$-type multiplicities in degenerate principal series via Howe duality

Let $K$ be one of the complex classical groups ${\rm O}_k$, ${\rm GL}_k$, or ${\rm Sp}_{2k}$. Let $M \subseteq K$ be the block diagonal embedding ${\rm O}_{k_1} \times \cdots \times {\rm O}_{k_r}$ or ${\rm GL}_{k_1} \times \cdots \times {\rm GL}_{k_r}$ or ${\rm Sp}_{2k_1} \times \cdots \times {\rm Sp}_{2k_r}$, respectively. By using Howe duality and seesaw reciprocity as a unified conceptual framework, we prove a formula for the branching multiplicities from $K$ to $M$ which is expressed as a sum of generalized Littlewood-Richardson coefficients, valid within a certain stable range. By viewing $K$ as the complexification of the maximal compact subgroup $K_{\mathbb{R}}$ of the real group $G_{\mathbb{R}} = {\rm GL}(k,\mathbb{R})$, ${\rm GL}(k, \mathbb{C})$, or ${\rm GL}(k,\mathbb{H})$, respectively, one can interpret our branching multiplicities as $K_{\mathbb{R}}$-type multiplicities in degenerate principal series representations of $G_{\mathbb{R}}$. Upon specializing to the minimal $M$, where $k_1 = \cdots = k_r = 1$, we establish a fully general tableau-theoretic interpretation of the branching multiplicities, corresponding to the $K_{\mathbb{R}}$-type multiplicities in the principal series.

==> Table_p.tex <==
\begin{tblr}{colspec={|Q[m,c]|Q[m,c]|Q[m,c]|Q[m,c]|},stretch=1.5}

\hline

$H$ & $r$ & $\widetilde{U}^0 \cong \C[W]^H \cong \begin{cases}
\C[\p^+], & k \geq r,\\
\C[\overline{\mathcal{O}}_k], & k < r
\end{cases}$ & Decomp.~as $\k$-module \\

\hline[2pt]

$\GL_k$ & 
$\min\{p,q\}$ & 
$\begin{cases}
    \C[\M_{p,q}]\\[1ex]
    \C\!\left[\M_{p,q}^{\leqslant k}\right]
\end{cases}$ & $\hspace{5ex}\displaystyle\bigoplus_{\mathclap{\substack{\nu:\\\ell(\nu) \leq \min\{k,r\}}}} F^\nu_p \otimes F^\nu_q$\\

\hline

$\O_k$ & 
$n$ & $\begin{cases} \C[{\rm SM}_{n}]\\[1ex]
\C\!\left[{\rm SM}_{n}^{\leqslant k}\right]
\end{cases}$ & $\displaystyle\bigoplus_{\mathclap{\substack{\nu:\\\ell(\nu) \leq \min\{k,r\},\\\text{$\nu$ has even rows}}}} F^\nu_n$\\

\hline

$\Sp_{2k}$ & 
$\lfloor n/2 \rfloor$ & $\begin{cases} \C[{\rm AM}_{n}]\\[1ex]
\C\!\left[{\rm AM}_{n}^{\leqslant 2k}\right]
\end{cases}$ & $\displaystyle\bigoplus_{\mathclap{\substack{\nu:\\\ell(\nu) \leq 2\min\{k,r\},\\\text{$\nu$ has even columns}}}} F^\nu_n$\\

\hline

\end{tblr}
